Instance-preserving graded semantic reporting for surgical action triplets

Complete-or-reject reporting of surgical action triplets can discard a correctly identified instrument and action when the target is uncertain. We introduce instance-preserving graded semantic reporting, which separates instance selection from the choice of semantic detail. Each selected instance retains its predicted mask and labels while hierarchical correctness scores guide instrument (I), instrument-verb (IV), or complete instrument-verb-target (IVT) reporting. The utility-increment rule DELTA weighs the expected gain from finer reporting against its error cost. We compare three decision rules on 5,641 test frames from eight surgical videos using fixed predictions and scores. At the 10% development calibration target, DELTA retains correct partial reports for 80.0% of candidates rejected by a matched complete-or-reject baseline (5,329/6,662). Adding IV increases source-normalized weighted correct-report yield by 19.13 to 23.13 per 100 frames across all three rules relative to separately recalibrated I/IVT controls. Weighted reporting risk changes by -0.77 to +1.01 percentage points, with complete correct-triplet counts unchanged or reduced. Graded reporting makes partial surgical predictions available as localized descriptions, with an explicit trade-off between report utility and completeness.

==> citation_commands.tex <==
% Load after natbib in the manuscript preamble. Keeps CAS bibliography sizing.
\RequirePackage{etoolbox}
\makeatletter
\DeclareRobustCommand{\APAand}{\ifNAT@swa\&\else and\fi}
% APA7 parenthetical groups follow the alphabetical bibliography order.
\def\NAT@sort{\@ne}
% Natbib normally shortens 2023a,2023b to 2023a,b. APA7 repeats each year.
% Patch the parenthetical and narrative branches independently, retaining links.
\patchcmd{\NAT@citex}
  {\NAT@hyper@{\NAT@exlab}}
  {\unskip\NAT@spacechar\NAT@hyper@{\NAT@date}}
  {}{\PackageError{eswa-apa7}{Cannot patch parenthetical year labels}{Check the natbib version.}}
\patchcmd{\NAT@citex}
  {\NAT@hyper@{\NAT@exlab}}
  {\unskip\NAT@spacechar\NAT@hyper@{\NAT@date}}
  {}{\PackageError{eswa-apa7}{Cannot patch narrative year labels}{Check the natbib version.}}
\makeatother
\setcitestyle{authoryear,round,semicolon,aysep={,},yysep={,}}

